A new class of Roche lobe-filling hot subdwarf binaries

We present the discovery of the second binary with a Roche lobe-filling hot subdwarf transferring mass to a white dwarf (WD) companion. This 56 minute binary was discovered using data from the Zwicky Transient Facility. Spectroscopic observations reveal an He-sdOB star with an effective temperature of $T_{\rm eff}=33,700\pm1000$ K and a surface gravity of $log(g)=5.54\pm0.11$. The GTC+HiPERCAM light curve is dominated by the ellipsoidal deformation of the He-sdOB star and shows an eclipse of the He-sdOB by an accretion disk as well as a weak eclipse of the WD. We infer a He-sdOB mass of $M_{\rm sdOB}=0.41\pm0.04$ M$_\odot$ and a WD mass of $M_{\rm WD}=0.68\pm0.05$ M$_\odot$. The weak eclipses imply a WD black-body temperature of $63,000\pm10,000$ K and a radius $R_{\rm WD}=0.0148\pm0.0020$ M$_\odot$ as expected for a WD of such high temperature. The He-sdOB star is likely undergoing hydrogen shell burning and will continue transferring mass for $\approx1$ Myrs at a rate of $10^{-9} M_\odot {\rm yr}^{-1}$ which is consistent with the high WD temperature. The hot subdwarf will then turn into a WD and the system will merge in $\approx30$ Myrs. We suggest that Galactic reddening could bias discoveries towards preferentially finding Roche lobe-filling systems during the short-lived shell burning phase. Studies using reddening corrected samples should reveal a large population of helium core-burning hot subdwarfs with $T_{\rm eff}\approx25,000$ K in binaries of 60-90 minutes with WDs. Though not yet in contact, these binaries would eventually come into contact through gravitational wave emission and explode as a sub-luminous thermonuclear supernova or evolve into a massive single WD.

==> ZTFJ2130+4420_photometry_results.tex <==

\begin{tabular}{lr}
\hline
%\hline
%Object: ZTFJ2130+4420 & 68\% confidence %interval\\
%\hline
%Color excess $E(B-V)$ from \href{https://ui.adsabs.harvard.edu/abs/1998ApJ...500..525S/abstract}{SFD (1998)} & $1.91\pm0.06$\,mag \\
%Color excess $E(B-V)$ from \href{https://ui.adsabs.harvard.edu/abs/2011ApJ...737..103S/abstract}{S\&F (2011)} & $1.64\pm0.05$\,mag \\
%\hline
Color excess $E(B-V)^{\text a}$ & $0.559\pm0.021$\,mag \\
%Extinction parameter $R(55)$ (fixed) & $3.02$ \\
Angular diameter $\log(\Theta\,\mathrm{(rad)})$ & $-11.479\pm0.011$ \\
%Absolute Magnitude $M_{\rm g}$   & $4.x\pm0.y$ [mag]  \\
%Parallax $\varpi$ ({\it Gaia}, $\text{RUWE}=0.93$) & $0.43\pm0.10$\,mas \\
%Effective temperature $T_{\mathrm{eff}}$ (prescribed) & $33700\pm1000$\,K \\
%Surface gravity $\log (g\,\mathrm{(cm\,s^{-2})})$ (prescribed) & $5.54\pm0.11$ \\
%Microturbulence $\xi$ (fixed) & $0$\,km\,s$^{-1}$ \\
%Metallicity $z$ (fixed) & $0$\,dex \\
%Helium abundance $\log(n(\textnormal{He}))$ (fixed) & $-0.3$ \\
Radius $R = \Theta/(2\varpi)$ & $0.17^{+0.05}_{-0.04}$\,$R_\odot$ \\
Mass $M = g R^2/G$ & $0.37^{+0.29}_{-0.14}$\,$M_\odot$ \\
Luminosity $L/L_\odot = (R/R_\odot)^2(T_\mathrm{eff}/T_{\mathrm{eff},\odot})^4$ & $34^{+24}_{-12}$ \\
%\hline
%Generic excess noise $\delta_\textnormal{excess}$ & $0.026$\,mag \\
%Reduced $\chi^2$ at the best fit & $1.00$ \\
%Parameter reference & Kupfer+ \\
\hline
\end{tabular}

